Pilot-Aided Distributed Multi-Group Multicast Precoding Design for Cell-Free Massive MIMO

We propose fully distributed multi-group multicast precoding designs for cell-free massive multiple-input multiple-output (MIMO) systems with modest training overhead. We target the minimization of the sum of the maximum mean squared errors (MSEs) over the multicast groups, which is then approximated with a weighted sum MSE minimization to simplify the computation and signaling. To design the joint network-wide multi-group multicast precoders at the base stations (BSs) and the combiners at the user equipments (UEs) in a fully distributed fashion, we adopt an iterative bi-directional training scheme with UE-specific or group-specific precoded uplink pilots and group-specific precoded downlink pilots. To this end, we introduce a new group-specific uplink training resource that entirely eliminates the need for backhaul signaling for the channel state information (CSI) exchange. The precoders are optimized locally at each BS by means of either best-response or gradient-based updates, and the convergence of the two approaches is analyzed with respect to the centralized implementation with perfect CSI. Finally, numerical results show that the proposed distributed methods greatly outperform conventional cell-free massive MIMO precoding designs that rely solely on local CSI.

==> authors_detials/Italo_bio.tex <==
Italo Atzeni received the MSc degree (Hons.) in telecommunications engineering from the University of Cagliari, Italy, in 2010 and the PhD degree (Hons.) in signal theory and communications from the Polytechnic University of Catalonia–BarcelonaTech, Spain, in 2014. Since 2019, he is with the Centre for Wireless Communications, University of Oulu, Finland, where he is currently an Assistant Professor and Academy Research Fellow. From 2014 to 2017, he was a Researcher at the Mathematical and Algorithmic Sciences Lab, Huawei Technologies, France. From 2017 to 2018, he was a Research Associate at EURECOM, France. He previously held a visiting research appointment at The Hong Kong University of Science and Technology, Hong Kong, in 2013. His primary research interests are in communication theory, signal processing, convex and distributed optimization theory, and their applications to low-complexity, energy-efficient solutions for multi-antenna communications. He received Best Paper Awards at IEEE ICC 2019 (Wireless Communications Symposium) and IEEE SPAWC 2023. He received the MSCA Individual Fellowship (2020–2022) by the European Commission and the Academy Research Fellowship (2022–2027) by the Research Council of Finland. He serves as an Editor for the IEEE Communications Letters.

==> authors_detials/antti_bio.tex <==
Antti Tölli (M'08, SM'14) is a Professor with the Centre for Wireless Communications (CWC), University of Oulu. He received the Dr.Sc. (Tech.) degree in electrical engineering from the University of Oulu, Oulu, Finland, in 2008. From 1998 to 2003, he worked at Nokia Networks as a Research Engineer and Project Manager both in Finland and Spain. In May 2014, he was granted a five year (2014-2019) Academy Research Fellow post by the Academy of Finland. During the academic year 2015-2016, he visited at EURECOM, Sophia Antipolis, France, while from August 2018 till June 2019 he was visiting at the University of California Santa Barbara, USA. He has authored numerous papers in peer-reviewed international journals and conferences and several patents all in the area of signal processing and wireless communications. His research interests include radio resource management and transceiver design for broadband wireless communications with a special emphasis on distributed interference management in heterogeneous wireless networks. From 2017 to 2021 he served as an Associate Editor for IEEE Transactions on Signal Processing.

==> authors_detials/bikshapathi_gouda_bio.tex <==
Bikshapathi Gouda received his master’s degree in communication systems from the Indian Institute of Technology Madras, India, in 2013. He is currently pursuing a Ph.D. degree with the Centre for Wireless Communications, University of Oulu, Finland. In 2013, he joined a startup company to work on the physical-layer design of 802.11ad WiFi technologies. In 2017, he moved to Cypress Semiconductor, India, to contribute to the development of 802.11ac/ax WiFi technologies. His research interests include communication theory, signal processing, convex optimization, and their application to distributed multiantenna systems and energy-efficient communications.

==> related_conference_publications.tex <==
Part of this work was presented at IEEE GLOBECOM 2022, which is listed in the references of the paper and also below:

[1] B. Gouda, I. Atzeni, and A. Tölli, “Distributed precoding design for multi-group multicasting in cell-free massive MIMO,” in Proc. IEEE
Global Commun. Conf. (GLOBECOM), Rio de Janeiro, Brazil, Dec.
2022.
